SAP: Corrective Machine Unlearning with Scaled Activation Projection for Label Noise Robustness

Label corruption, where training samples are mislabeled due to non-expert annotation or adversarial attacks, significantly degrades model performance. Acquiring large, perfectly labeled datasets is costly, and retraining models from scratch is computationally expensive. To address this, we introduce Scaled Activation Projection (SAP), a novel SVD (Singular Value Decomposition)-based corrective machine unlearning algorithm. SAP mitigates label noise by identifying a small subset of trusted samples using cross-entropy loss and projecting model weights onto a clean activation space estimated using SVD on these trusted samples. This process suppresses the noise introduced in activations due to the mislabeled samples. In our experiments, we demonstrate SAP's effectiveness on synthetic noise with different settings and real-world label noise. SAP applied to the CIFAR dataset with 25% synthetic corruption show upto 6% generalization improvements. Additionally, SAP can improve the generalization over noise robust training approaches on CIFAR dataset by ~3.2% on average. Further, we observe generalization improvements of 2.31% for a Vision Transformer model trained on naturally corrupted Clothing1M.

==> content/80_backup_old_results.tex <==


\iffalse
\begin{table}[b]
\caption{ Test Accuracy for symmetric noise (Equation~\ref{eqn:sym_noise}) removal from CIFAR10 and CIFAR100 datasets trained on VGG11 and ResNet18 architectures with noise strength $\eta=0.1$ and $\eta=0.25$. We report the mean and standard deviation across three randomly chosen seeds.
% Verifix and Finetune methods use 1000 trusted samples. 
%See Appendix~\ref{apx:low_syn_noise} in Supplementary Material for a lower level of synthetic noise. 
} \label{tab:sym_cifar}
\begin{center}
\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{l|l|cc|cc}
\Xhline{3\arrayrulewidth}
& \multirow{2}{*}{\bf Method}  & \multicolumn{2}{c|}{\bf \texttt{VGG11\_BN}} &  \multicolumn{2}{c}{\bf \texttt{ResNet18}}\\
%&&  \multicolumn{2}{c|}{\bf Percentage Mislabeled Samples} &  \multicolumn{2}{c}{\bf Percentage Mislabeled Samples}\\
&& {\bf $\eta=0.1$}& {\bf $\eta=0.25$}& {\bf $\eta=0.1$}& {\bf $\eta=0.25$}\\
    \hline  
\Xhline{3\arrayrulewidth}
    \multirow{5}{*}{\bf \rotatebox[origin=c]{90}{CIFAR10}}
        %& Ideal     &  \multicolumn{2}{c|}{$90.94\pm0.27$}
        %            &  \multicolumn{2}{c}{$93.48\pm0.18$}\\
        & Retrain   & $90.18\pm0.14$ & $89.48\pm0.04$
                    & $93.21\pm0.22$ & $92.45\pm0.06$\\ 
        \cline{2-6}
        & Vanilla   & $86.04\pm0.17$& $76.69\pm0.46$
                    & $88.54\pm0.16$& $79.47\pm0.46$\\  
        & Finetune   &$\pm$ & $\pm$ 
                    & $\pm$ & $\pm$ \\
        & SSD       &$\pm$ & $\pm$ 
                    & $\pm$ & $\pm$ \\
        & SAP       & $87.44\pm0.46$& $82.707\pm0.20$
                    & $90.08\pm0.17$ &$85.48\pm0.36$\\
\Xhline{3\arrayrulewidth}
    \multirow{5}{*}{\bf \rotatebox[origin=c]{90}{CIFAR100}}
        %& Ideal     &  \multicolumn{2}{c|}{$66.79\pm0.27$}
        %            &  \multicolumn{2}{c}{$73.56\pm0.17$}\\
        & Retrain   & $65.76\pm0.23$& $63.66\pm0.49$ 
                    & $73.56\pm0.48$&$72.13\pm0.36$\\
        \cline{2-6}
        & Vanilla   & $60.66\pm0.23$& $49.03\pm0.69$ 
                    & $68.16\pm0.40$&$54.76\pm0.45$\\
        & Finetune  &$\pm$ & $\pm$ 
                    & $\pm$ & $\pm$ \\
        & SSD       &$\pm$ & $\pm$ 
                    & $\pm$ & $\pm$ \\
        & SAP       & $61.32\pm0.09$& $53.507\pm0.89$ 
                    & $66.73\pm0.15$ &$58.77\pm0.63$\\ 
\Xhline{3\arrayrulewidth}
\end{tabular}
}
\end{center}
%\end{table}
%\begin{table}[b]
\caption{ Test Accuracy for asymmetric noise (Equation~\ref{eqn:asym_noise}) and Hierarchical noise (Equation~\ref{eqn:real_noise})  removal from CIFAR10 and CIFAR100 datasets trained on ResNet18 architecture with noise strength of $\eta=0.25$. We report the mean and standard deviation across three randomly chosen seeds.
% Verifix and Finetune methods use 1000 trusted samples. 
%See Appendix~\ref{apx:low_syn_noise} in Supplementary Material for a lower level of synthetic noise. 
} \label{tab:asym_real_cifar}
\begin{center}
\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{l|l|cc|cc}
\Xhline{3\arrayrulewidth}
& \multirow{2}{*}{\bf Method}  & \multicolumn{2}{c|}{\bf \texttt{Asymmetric Noise}} &  \multicolumn{2}{c}{\bf \texttt{Hierarchical Noise}}\\
%&&  \multicolumn{2}{c|}{\bf Percentage Mislabeled Samples} &  \multicolumn{2}{c}{\bf Percentage Mislabeled Samples}\\
&& {\bf $\eta=0.1$}& {\bf $\eta=0.25$}& {\bf $\eta=0.1$}& {\bf $\eta=0.25$}\\
    \hline  
\Xhline{3\arrayrulewidth}
    \multirow{5}{*}{\bf \rotatebox[origin=c]{90}{CIFAR10}}
        %& Ideal     &  \multicolumn{2}{c|}{$90.94\pm0.27$}
        %            &  \multicolumn{2}{c}{$93.48\pm0.18$}\\
        & Retrain   & $90.18\pm0.14$ & $89.48\pm0.04$
                    & $93.21\pm0.22$ & $92.45\pm0.06$\\ 
        \cline{2-6}
        & Vanilla   & $86.04\pm0.17$& $76.69\pm0.46$
                    & $88.54\pm0.16$& $79.47\pm0.46$\\  
        & Finetune   &$\pm$ & $\pm$ 
                    & $\pm$ & $\pm$ \\
        & SSD       &$\pm$ & $\pm$ 
                    & $\pm$ & $\pm$ \\
        & SAP       & $87.44\pm0.46$& $82.707\pm0.20$
                    & $90.08\pm0.17$ &$85.48\pm0.36$\\
\Xhline{3\arrayrulewidth}
    \multirow{5}{*}{\bf \rotatebox[origin=c]{90}{CIFAR100}}
        %& Ideal     &  \multicolumn{2}{c|}{$66.79\pm0.27$}
        %            &  \multicolumn{2}{c}{$73.56\pm0.17$}\\
        & Retrain   & $65.76\pm0.23$& $63.66\pm0.49$ 
                    & $73.56\pm0.48$&$72.13\pm0.36$\\
        \cline{2-6}
        & Vanilla   & $60.66\pm0.23$& $49.03\pm0.69$ 
                    & $68.16\pm0.40$&$54.76\pm0.45$\\
        & Finetune  &$\pm$ & $\pm$ 
                    & $\pm$ & $\pm$ \\
        & SSD       &$\pm$ & $\pm$ 
                    & $\pm$ & $\pm$ \\
        & SAP       & $61.32\pm0.09$& $53.507\pm0.89$ 
                    & $66.73\pm0.15$ &$58.77\pm0.63$\\ 
\Xhline{3\arrayrulewidth}
\end{tabular}
}
\end{center}
\end{table}

\subsubsection{Results :}
Our results in Table~\ref{tab:mislabel_cifar_sam} show the Retrain models perform closely match the Ideal model, indicating that mildly reducing dataset size has minimal impact on model generalization \cite{guo2022deepcore}. 
In contrast, the Vanilla model experiences a significant drop in test accuracy, especially at higher noise levels. 
We observe a $15-20\%$ drop with $25\%$ corruption level for both CIFAR10 and CIFAR100. 
This highlights the severe impact of label noise on performance.  
Finetuning the Vanilla model on a small set of trusted samples (1000 for 50 epochs) consistently improves performance. 
Notably, finetuning on just 1000 samples can boost performance by approximately $8\%$ for a VGG11 model trained on CIFAR10 with $25\%$ corruption (see Finetune in Table~\ref{tab:mislabel_cifar_sam}). 
Applying our method to the Vanilla model (Verifix\textsubscript{Vanilla}) leads to significant improvements on both CIFAR10 and CIFAR100 datasets.
With a  $25\%$ corruption rate, we observe gains of $11.19\%$ (VGG11) and $6.97\%$  (ResNet18) on CIFAR10, 
 and  $7.78\%$ (VGG11) and $3.5\%$ (ResNet18) on CIFAR100. 
%In our experiments, we found that combining our method with finetuning did not yield further generalization benefits. 
\begin{table*}[t]
\caption{ Test Accuracy for label noise removal on CIFAR10 and CIFAR100 datasets trained on VGG11 and ResNet18 architectures with $10\%$ and $25\%$ label corruption. We report the mean and standard deviation across three randomly chosen seeds.
Verifix and Finetune methods use 1000 trusted samples. See Appendix~\ref{apx:low_syn_noise} in Supplementary Material for a lower level of synthetic noise. } \label{tab:mislabel_cifar_sam}
\begin{center}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|l|cc|cc}
 \hline
& \multirow{3}{*}{\bf Method}  & \multicolumn{2}{c|}{\bf \texttt{VGG11\_BN}} &  \multicolumn{2}{c}{\bf \texttt{ResNet18}}\\
&&  \multicolumn{2}{c|}{\bf Percentage Mislabeled Samples} &  \multicolumn{2}{c}{\bf Percentage Mislabeled Samples}\\
&& {\bf 10\%}& {\bf 25\%}& {\bf 10\%}& {\bf 25\%}\\
    \hline  \hline 
    \multirow{7}{*}{\bf \rotatebox[origin=c]{90}{CIFAR10}}
        & Ideal &  \multicolumn{2}{c|}{$91.18\pm0.17$}&  \multicolumn{2}{c}{$94.23\pm0.06$}\\
        & Retrain & $90.73\pm0.15$ & $89.60\pm0.21$
                  & $93.77\pm0.25$ & $93.08\pm0.21$\\
        & Vanilla  & $85.01\pm0.38$& $72.19\pm0.33$
                   & $88.66\pm0.38$& $78.37\pm0.18$\\    
        & SAM & $\textbf{89.96}\pm\textbf{0.1}$& $87.05\pm0.28$
                  & $90.80\pm0.13$& $83.76\pm0.11$\\
        & Finetune  &$87.03\pm0.42$ & $81.82\pm0.25$ 
                                   & $89.49\pm0.2$ & $82.82\pm0.70$ \\
        & Verfix\textsubscript{Vanilla} & $87.78\pm0.18$& $83.38\pm0.47$
                                                & $90.46\pm0.10$ &$86.96\pm0.14$\\
        & Verfix\textsubscript{SAM}  & $89.95\pm0.11$& $\textbf{87.17}\pm\textbf{0.38}$ 
                                                & $\textbf{91.42}\pm\textbf{0.14}$ &$\textbf{87.74}\pm\textbf{0.38}$\\
\hline
    \multirow{7}{*}{\bf \rotatebox[origin=c]{90}{CIFAR100}}
        & Ideal &  \multicolumn{2}{c|}{$67.44\pm0.18$}&  \multicolumn{2}{c}{$75.34\pm0.06$}\\
        & Retrain   & $65.99\pm0.43$& $63.73\pm0.52$ 
                    & $73.89\pm0.16$&$72.13\pm0.36$\\
        
        
        & Vanilla   & $60.66\pm0.23$& $49.03\pm0.69$ 
                    & $68.16\pm0.40$&$57.60\pm0.17$\\
        & SAM & $62.58\pm0.52$& $54.31\pm0.21$
                  & $69.64\pm0.18$& $58.82\pm0.76$\\
        & Finetune & $60.68\pm0.23$ & $49.01\pm0.70$ 
                    & $68.42\pm0.53$ & $58.67\pm0.17$ \\
        & Verfix\textsubscript{Vanilla}   & $63.10\pm0.40$& $56.81\pm0.37$ & 
                                                 $69.16\pm0.16$ &$61.42\pm0.46$\\
        & Verfix\textsubscript{SAM} & $\textbf{63.80}\pm\textbf{0.50}$& $\textbf{58.33}\pm\textbf{0.11}$
                                                & $\textbf{70.21}\pm\textbf{0.16}$ &$\textbf{62.19}\pm\textbf{0.66}$\\
 \hline
\end{tabular}
}
\end{center}
\end{table*}

%% Robust training
We compare our approach to SAM \cite{foret2021sharpnessaware},  which is a training technique more robust to label noise but requires double the resources of standard SGD. 
While SAM s more robust to label noise over the Vanilla model, our method applied to the Vanilla model (Verifix\textsubscript{Vanilla} in Table~\ref{tab:mislabel_cifar}) outperforms SAM in most cases with $25\%$ corruption and remains competitive at $10\%$ corruption. 
The only exception is VGG11 on CIFAR10, where SAM shows slightly higher gains ($2.18\%$ at $10\%$ corruption, $3.67\%$ at $25\%$). 
Importantly, Verfix\textsubscript{Vanilla} demonstrates an average improvement of $0.58\%$ over SAM, highlighting its effectiveness while requiring significantly fewer computational resources.
Additionally, applying our method to SAM-trained models (Verifix\textsubscript{SAM} in Table~\ref{tab:mislabel_cifar_sam}) further boosts accuracy up to $4.02\%$, achieving the best results in  Table~\ref{tab:mislabel_cifar_sam}. 
This highlights that our method is complementary to existing noise-robust training techniques, offering additional generalization improvements.
\begin{figure*}[t]
\centering
    \begin{minipage}{.31\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{content/images/sample_selection_cifar100_all.pdf}
        \caption{Effect of sampling strategy on CIFAR100 dataset for model trained with $25\%$ corrupt labels.}
        \label{fig:sampling_strategy}
    \end{minipage}
    \quad 
    \begin{minipage}{.31\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{content/images/sample_size_cifar100_all.pdf}
        \caption{Effect of trusted sample size on CIFAR100 dataset for model trained with $25\%$ corrupt labels.}
        \label{fig:sample_size}
    \end{minipage}
    \quad
    \begin{minipage}{.31\textwidth}
        \centering
        \includegraphics[width=.9\linewidth]{content/images/alpha_all_all.pdf}
        \caption{Effect of $\alpha$ for model trained with $25\%$ corrupt labels.}
        \label{fig:alpha_effect}
    \end{minipage} 
\end{figure*}
\subsection{Analyses}
\subsubsection{Selecting samples with low curvature improves generalization :}

Our approach uses a few trusted samples from the clean portion of the training dataset ($\mathcal{D}^{cln}_{Tr}$).
We explored six different sampling strategies in Figure~\ref{fig:sampling_strategy}.
The \textit{Expert} strategy provides 1000 correctly labeled samples from $\mathcal{D}^{cln}_{Tr}$, requiring access to ground-truth labels.
Alternatively, we use curvature scores (Equation~\ref{eqn:curvature}) to identify likely clean samples from the corrupted dataset $\mathcal{D}^{cpt}_{Tr}$.
We sort samples by ascending curvature and select 1000 based on percentile scores (\textit{0\%, 10\%, 25\%, 50\%} strategy) or random sampling from the lower \textit{50\%} percentile samples (\textit{Uniform} strategy). 
By \textit{x\%} sampling strategy, we mean selecting 1000 images after the $x^{th}$ percentile of low-curvature samples.
Interestingly, selecting the 1000 lowest curvature samples (\textit{0\%} sampling) consistently outperforms other strategies, suggesting these samples are most beneficial for our method.
For CIFAR100 dataset with \textit{0\%} sampling, we achieve $56.85\%$ and $61.1\%$ test accuracy on VGG11 and ResNet18 model, respectively.
We observe that performance decreases as we sample from higher curvature percentiles, with steeper declines for VGG11.
Our experiments show an curvature based sampling improves the generalization up to $1.06\%$ for \textit{0\%} strategy when compared to \textit{Expert}.
Additionally, the \textit{Expert} sampling strategy gives similar performance to \textit{Unifrom} strategy ($\sim55.8\%$ for VGG11 and $\sim60.55\%$ for ResNet18 on CIFAR100).

\subsubsection{Increasing Trusted Sample Size yields diminishing returns in performance :}
We study how the number of trusted samples impacts our method's performance and computational cost. 
Since representation calculations and SVD are performed on the trusted set, the sample size directly affects compute requirements. 
Figure~\ref{fig:sample_size} shows how test accuracy varies with the number of trusted samples. 
We observe that increasing the sample size improves accuracy up to 1000 samples, after which there are no significant gains.  
Therefore, we use 1000 samples in our experiments to balance performance and computational efficiency.



\subsubsection{Finding the optimal scaling hyperparameter ($\alpha$) is key to maximizing performance gains :}
Figure~\ref{fig:alpha_effect} demonstrates how the scaling factor ($\alpha$) influences test accuracy for models trained on datasets with $25\%$ label corruption. We observe that increasing $\alpha$ generally improves test accuracy up to a certain point, after which accuracy gradually declines. 
Importantly, we find that $\alpha=30000$ consistently yields strong results across different datasets, models, and corruption levels. 




 \begin{figure*}
\centering
 \begin{minipage}{.34\textwidth}    
            \centering
            \includegraphics[width=0.98\textwidth]{content/images/compute_cifar100_resnet18.pdf}
            \captionof{figure}{Compute comparisons for several methods for ResNet18 model trained on CIFAR100 dataset.}
            \label{fig:compute}
    \end{minipage}
  \hfill
  \begin{minipage}{0.6\textwidth}
    \centering
      \captionof{table}{Generalization benefits of applying our algorithm in synergy with noise-robust training approaches on real-world datasets including Mini-WebVision\cite{mentormix}, WebVision1.0\cite{li2017webvision}, and Clothing1M\cite{xiao2015learning}. \textbf{Metrics}: Validation accuracy for Mini-WebVision and WebVision1.0, Test accuracy for Clothing1M. \label{tab:real_noise}} 
      
        \resizebox{0.95\textwidth}{!}{
                \begin{tabular}{l|l|c|c}
                 \hline
                    \multirow{2}{*}{\bf Dataset (Network)} & \multirow{2}{*}{\bf  Method}  & {\bf Baseline} &{\bf Verifix Accuracy} \\
                    &&{\bf Accuracy}&{\bf (Improvements)}\\
                    \hline  \hline 
                        & Vanilla & $63.81\pm0.38$ &  $64.96\pm0.53$ ($+1.15$)\\
                        Mini-WebVision \cite{mentormix} & MixUp\cite{mixup} & $65.02\pm0.40$ & $\textbf{66.21}\pm\textbf{0.58 (+1.2)}$\\
                        (InceptionResNetV2)& MentorMix\cite{mentormix} & $65.34\pm0.65$  & $65.76\pm0.88$  ($+0.88$) \\
                        & SAM\cite{foret2021sharpnessaware} & $65.68\pm0.57$ & $66.10\pm0.46$ ($+0.46$)\\
                        \hline
                        WebVision1.0 \cite{li2017webvision}& \multirow{2}{*}{Vanilla} & \multirow{2}{*}{$64.86\pm0.53$}&\multirow{2}{*}{$\textbf{65.26}\pm\textbf{0.49 (+0.40)}$}\\
                        (InceptionResNetV2)&&&\\
                        \hline
                        Clothing1M \cite{xiao2015learning}& Vanilla & $67.48\pm0.63$  & $\textbf{70.11}\pm\textbf{0.76 (+2.63)}$\\
                        (ResNet50)& MixUp & $67.89\pm0.63$ & $69.84\pm1.16$ ($+1.94$)\\
                    \hline
                    \hline 
                    \multicolumn{2}{c|}{\bf Average}&$65.73$&$\textbf{66.85}$ ($+1.13$)\\
                    \hline
                \end{tabular}
            }
    
    \end{minipage}
  \end{figure*}
\subsubsection{Verifix achieves SAM-level performance at a fraction of the computational cost : }
We analytically evaluate the computational cost of different methods in Figure~\ref{fig:compute}. 
In our evaluations, we only consider the convolution and linear layers and ignore the compute for normalization, pooling, and non-linearities in the network. 
Compute of forward pass for linear layer is $n_{sample} f_{in} f_{out}$, where $n_{sample}$ is the number of samples, $f_{in}$ is the input dimension of linear layer and $f_{out}$ is the output dimension. 
For a convolutional layer with a kernel of size $C_{in}\times k \times k \times C_{out}$ producing an output map of size $h_o\times w_o$ requires compute of $n_{sample}h_ow_oC_{in}k^2C_{out}$ for the forward pass. 
The backward pass cost is approximated as twice the forward pass cost.  
Note, here $n_{samples}$ is the effective number of samples seen during the training or finetuning. If a model is trained for 50 epochs with 1000 samples in each epoch, then the value for $n_{sample}$ is 50000.
This explains the analytical compute costs for Finetune, Retrain, and Ideal baselines, which use standard SGD. 
SAM, requiring two forward and backward passes per iteration, has its compute cost approximated by doubling the SGD cost.


We decompose Verifix's computation into five steps: Trusted sample Estimation, Representation Sampling, SVD, Space Estimation, and Weight Projection. 
Trusted Sample Estimation involves a few gradient computation epochs ( $\sim10$) over $\mathcal{D}_{Tr}^{cpt}$  using curvature estimation \cite{garg2023memorization}. 
Representation Sampling requires a forward pass on the trusted sample set. 
SVD cost for an m×n matrix (where $m>n$) is approximately $mn^2$ \cite{cline2006computation}. 
Space Estimation and weight projection primarily involve matrix multiplications,  where the cost for multiplying an $m\times n$ matrix with an $n\times p$ matrix is $mnp$.
This analytical framework, including the previously discussed forward pass and matrix multiplication costs, explains the compute estimates in Figure~\ref{fig:compute}. 
The bar plot in Figure~\ref{fig:compute} displays these analytical compute estimates on a log scale, with bar labels indicating normalized compute values relative to Verifix.
Verifix demonstrates performance competitive to SAM (see Table~\ref{tab:mislabel_cifar_sam}) while requiring significantly lower computational resources (Figure~\ref{fig:compute}). 
Particularly, the total compute requirement for Verifix applied to a Vanilla model is less than $\sim51.5\%$ (calculated as $100\times(34.7+1)/69.4$) of the compute needed by SAM. 
This highlights Verifix's efficiency advantage without compromising accuracy.


\subsection{Real World Noise}
% Experiment 
To demonstrate our method's effectiveness in real-world noise scenarios, we present experiments on Mini-WebVision \cite{mentormix}, WebVision1.0 \cite{li2017webvision}, and Clothing1M \cite{xiao2015learning} datasets. 
Mini-WebVision and WebVision1.0 utilize the InceptionResNetV2 \cite{szegedy2017inception} architecture, while Clothing1M employs ResNet50 \cite{he2016deep}.  Comprehensive training and hyperparameter details are provided in Appendix~\ref{apx:training_details} in Supplementary Material.
In Table~\ref{tab:real_noise}, we establish several baselines for these datasets including Vanilla, MixUp \cite{mixup}, MentorMix \cite{mentormix}, and SAM \cite{foret2021sharpnessaware}. Following previous works, we report validation accuracy for Mini-WebVision and WebVision, and test accuracy for Clothing1M.


\subsubsection{Results :}
As shown in Table~\ref{tab:real_noise}, applying Verifix in conjunction with each of the noise-robust training methods consistently yields generalization improvements. These results demonstrate an average improvement of $1.13\%$, highlighting Verifix's ability to complement existing approaches while maintaining computational efficiency.  Importantly, our success with such larger datasets (containing millions of images), underscores the scalability of our method.
\fi

==> content/80_backup_related.tex <==
\section{Related Work}
\label{sec:related}
\iffalse
%Large-scale learning datasets are typically labeled by humans \cite{deng2009imagenet} and there are pervasive labeling errors in common machine learning datasets \cite{northcutt2021pervasive}. To address this challenge, 
We survey existing works in two key domains of label noise research:

\subsubsection{Data Cleaning (Domain 1) :} 
This direction of research focuses on detecting and correcting or removing mislabeled samples within the training dataset, ensuring the model only learns from accurately labeled data. 
The naive human (expert) in the loop relabeling is tedious and often error-prone \cite{sambasivan2021everyone}. 
In response, the research in this domain primarily focuses on the automatic detection of mislabeled samples. 
Several works \cite{feng2020label,brodley1999identifying,verbaeten2003ensemble,guo2014ensemble,sluban2014ensemble,zhu2003eliminating,khoshgoftaar2005enhancing} train an ensemble of models to filter out the incorrectly labeled samples.
%These approaches often employ either majority or consensus filters. A majority filter requires more than half of the classifiers to mispredict a label for the sample to be considered mislabeled, providing aggressive noise removal but risking the removal of difficult yet correctly labeled samples \cite{feng2020label}. A consensus filter, where only one classifier needs to mispredict, is less aggressive but also potentially retains some noise in the filtered datasets.
A major limitation of these ensemble-based approaches is their computational expense, especially for large datasets where training multiple models can be infeasible.
To address this challenge, several studies have focused on leveraging training dynamics to identify label noise, including methods such as using cross-validation on noisy splits \cite{chen2019understanding}, learning time \cite{liu2020early,xia2020robust}, forgetting time \cite{maini2022characterizing}, train-set confidence \cite{northcutt2021confident} or thorough input loss curvature \cite{garg2023memorization,ravikumar2024unveiling}.
While these approaches reduce computational overheads compared to ensemble-based methods, a remaining challenge lies in distinguishing between truly difficult examples and those that are mislabeled \cite{garg2023memorization}.
Additionally, approaches in this domain still necessitate retraining models on the filtered dataset, failing to fully leverage the models learned on the initial noisy data.
In contrast, our proposed Post-Training Correction paradigm seeks computationally efficient ways to directly adjust the corrupted model. 
This approach is crucial for large datasets and models where retraining might be computationally intractable.

\subsubsection{Noise-Robust Training (Domain 2) :}
This domain of algorithms tackles the challenge of label noise through the development of training techniques and loss functions that are inherently less sensitive to mislabeled data.  
Regularization techniques, such as dropout \cite{jindal2016learning} (which introduces randomness during training) and label smoothing \cite{lukasik2020does,wei2021smooth} (which softens target labels), help prevent overfitting and improve label noise robustness.  
Robust loss functions like symmetric cross-entropy \cite{wang2019symmetric} and Mean Absolute Error (MAE) reduce the impact of noisy labels compared to standard cross-entropy loss. 
Optimization methods like Sharpness-Aware Minimization (SAM) \cite{foret2021sharpnessaware} promote flatter loss landscapes, which are associated with better generalization under label noise. 
Additionally, curriculum and self-paced learning \cite{jiang2018mentornet,zhang2018generalized} gradually increase the difficulty of training examples, helping the model learn robust features before encountering noise. 
Data augmentation and mixup techniques (e.g., MixUp \cite{mixup}, DivideMix \cite{Li2020DivideMix}, MentorMix\cite{mentormix}) smooth training distributions, encouraging less abrupt decision boundaries and further enhancing robustness. 
While these robust algorithms offer improvement over standard training, they still have limitations. 
Some can be computationally expensive to implement or may reduce performance on clean datasets. Additionally, they often underperform compared to models trained with perfectly labeled data. Our proposed algorithm is orthogonal to these techniques and can be used in combination to further close this generalization gap.


%%\subsubsection{Post-Training Correction (Proposed) :}
%%
\fi
